Krylov Methods are (nearly) Optimal for Low-Rank Approximation

We consider the problem of rank-$1$ low-rank approximation (LRA) in the matrix-vector product model under various Schatten norms: $$ \min_{\|u\|_2=1} \|A (I - u u^\top)\|_{\mathcal{S}_p} , $$ where $\|M\|_{\mathcal{S}_p}$ denotes the $\ell_p$ norm of the singular values of $M$. Given $\varepsilon>0$, our goal is to output a unit vector $v$ such that $$ \|A(I - vv^\top)\|_{\mathcal{S}_p} \leq (1+\varepsilon) \min_{\|u\|_2=1}\|A(I - u u^\top)\|_{\mathcal{S}_p}. $$ Our main result shows that Krylov methods (nearly) achieve the information-theoretically optimal number of matrix-vector products for Spectral ($p=\infty$), Frobenius ($p=2$) and Nuclear ($p=1$) LRA. In particular, for Spectral LRA, we show that any algorithm requires $\Omega\left(\log(n)/\varepsilon^{1/2}\right)$ matrix-vector products, exactly matching the upper bound obtained by Krylov methods [MM15, BCW22]. Our lower bound addresses Open Question 1 in [Woo14], providing evidence for the lack of progress on algorithms for Spectral LRA and resolves Open Question 1.2 in [BCW22]. Next, we show that for any fixed constant $p$, i.e. $1\leq p =O(1)$, there is an upper bound of $O\left(\log(1/\varepsilon)/\varepsilon^{1/3}\right)$ matrix-vector products, implying that the complexity does not grow as a function of input size. This improves the $O\left(\log(n/\varepsilon)/\varepsilon^{1/3}\right)$ bound recently obtained in [BCW22], and matches their $\Omega\left(1/\varepsilon^{1/3}\right)$ lower bound, to a $\log(1/\varepsilon)$ factor.

==> reduction_to_block_krylov.tex <==
\section{Lower bound against Arbitrary Adaptive Algorithms}

In this section, we show that for a wide class of matrix-vector problems, it suffices to prove a lower bound against block Krylov algorithms. This will lead to an optimal lower bound for rank-1 spectral low-rank approximation, against an arbitrary adaptive algorithm.

Let $A = U^\top D U$, where $D$ is a (possibly random) diagonal matrix, $U$ is a Haar-random orthogonal matrix (see Definition~\ref{def:haar-random}), and $U$ and $D$ are independent. We consider the following model, which is a strengthening of the matrix-vector product model:

\begin{definition}[Extended Oracle Model]
\label{def:extended-oracle-model}
Given $K \in \mathbb{N}$, for all  $k \in [K]$, the algorithm chooses a new query point $v_k$, and receives the information $\{A^i v_j\}_{(i, j) \in H_k},$ where $H_k := \{(i, j): i+j \le k+1, i \ge 0, 1 \le j \le k\}$ is a set of ordered pairs of nonnegative integers. We use the following notation $\{A^i v_j\}_{S}$ for any set $S$ to denote $\{A^i v_j\}_{(i, j) \in S}$.  
\end{definition}


Note that this is clearly a stronger oracle model than before, so a lower bound against algorithms in the extended oracle model implies a lower bound against algorithms in the original matrix-vector model.

\begin{definition}[Adaptive Deterministic Algorithm]
\label{def:adaptive-deterministic-algorithm}
An \textit{adaptive deterministic algorithm} $\calA$ that makes $K$ extended oracle queries (see Def~\ref{def:extended-oracle-model}) is given by a deterministic collection of functions $v_1,v_2\Paren{\cdot},\dotsc,v_{K}\Paren{\cdot}$, where $v_1$ is constant and each $v_k \Paren{\cdot}$ is a function of $\frac{k\,(k+1)}{2}-1$ inputs.
This corresponds to a sequence of queries where the $k$-th query $v_k(\{A^i v_j\}_{H_{k-1}})$ is chosen adaptively based on the information available to the algorithm at the start of iteration $k$.
(Note that $v_1$ has no inputs.)
%$v_1$, $v_2(x_{0,1}, x_{1,1})$, \dots, $v_K(\{x_{i,j}\}_{i+j\le K, j<K})$, where $v_1$ is a deterministic unit vector, and for $k > 1$, $v_k$ is a vector-valued function that takes $\frac{k(k+1)}{2}-1$ vector inputs $\{x_{i,j}\}_{i+j\le k, j<k}$, and returns a \textit{deterministic unit vector that is orthogonal to all of $\{x_{i,j}\}_{i+j\le k, j<k}$}.
When the choice of the inputs is clear from context, we may simply write $v_k = v_k(\{A^i v_j\}_{H_{k-1}})$ for simplicity.
\end{definition}

In the extended oracle model, we can assume that each $v_k$ is a unit vector orthogonal to its inputs.
\begin{lemma}[Extended Oracle and Orthogonal Queries]
\label{lem:extended-oracle-queries-are-orthogonal}
For $k \in [2, K]$, let $v_k$ be as stated in Definition~\ref{def:adaptive-deterministic-algorithm} and let $\Set{A^{i} v_j }_{H_{k-1}}$ be as stated in Definition~\ref{def:extended-oracle-model}. Then, we may assume WLOG that $v_k$ is orthogonal to the subspace spanned by the vectors in $\Set{A^{i} v_j }_{H_{k-1}}$. 
\end{lemma}
\begin{proof}
Assume for sake of contradiction that this were not the case. Then, we can decompose $v_k = \sum_{(i, j) \in H_{k-1}} c_{i,j} A^i v_j + c^\perp v_k^\perp$ where $v_k^\perp$ is a unit vector orthogonal to $\{A^i v_j\}_{H_{k-1}}$ and each $c_{i, j}$ and $c^\perp$ is a scalar.
At the end of iteration $k$, the new information obtained by the algorithm is $\{A^i v_j\}_{i+j=k+1, j \le k}$.
For all $(i,j) \ne (1,k)$, the new information does not depend on $v_k$.
Also, $A v_k = \sum_{(i, j) \in H_{k-1}} c_{i,j} A^{i+1} v_j + c^\perp A v_k^\perp$, where each $A^{i+1} v_j$ is information obtained by the algorithm at the end of iteration $k+1$ regardless (due to our extended query model).
Since $(i+1, j) \in H_k$ if $(i, j) \in H_{k-1}$, and since $(1, k) \in H_k$, this expression shows that the algorithm would receive the same amount of information (or more, if $c^\perp = 0$) if it queries $v_k^\perp$ instead of $v_k$.
Applying this reasoning inductively proves the claim.
\end{proof}


%because if we had a function $\hat v_k(\{x_{i,j}\}_{i+j\le k, j<k})$ such that the output $\hat v_k$ is not orthogonal to $\{x_{i,j}\}_{i+j\le k, j<k}$, then we can always write $\hat v_k = \hat v_k^\perp + \hat v_k^\parallel$, where $\hat v_k^\perp$ is the component of $\hat v_k$ orthogonal to $\{x_{i,j}\}_{i+j\le k, j< k}$, and define $v_k(\{x_{i,j}\}_{i+j\le k, j<k})$ to be the unit vector parallel to $\hat v_k(\{x_{i,j}\}_{i+j\le k, j<k})^\perp$. Because an oracle query is linear in its inputs, the algorithms that use queries $v_k$ and $\hat v_k$ respectively will be equivalent.

We compare to a Block Krylov algorithm that makes i.i.d.\ standard Gaussian queries $z_1,z_2,\dotsc,z_K$ and then receives $\{A^i z_j\}$ for all $i, j \le K$. Recall, the Block Krylov algorithm does not make \emph{adaptive} queries, it is easier to prove lower bounds against Block Krylov algorithms. Our goal is to now show that Block Krylov algorithms can simulate an Adaptive Deterministic Algorithm.

\subsection{Conditioning lemma}\label{scn:conditioning}

We start by proving a general conditioning lemma which will be invoked repeatedly in the reduction to Block Krylov algorithms.
We implicitly assume that all mappings are measurable, in order to avoid undue technical issues. This lemma roughly shows that if the adaptive algorithm knows $\{A^i v_j\}_{H_k},$ the posterior distribution of $A$ given $\{A^i v_j\}_{H_k}$ is indeed rotationally symmetric on the orthogonal complement $\{A^i v_j\}_{H_k}$.

We will use the notation $\eqdist$ to denote that two random variables are equal in probability distribution (possibly conditioned on other information).

%For each integer $k \ge 0$, define $H_k$ to be the set of pairs of nonnegative integers $\{(i, j): i+j \le k+1, j \le k\}$.

\begin{lemma} \label{lem:random_rotation_fixed_subspace}
    Let $U$ be a Haar-random orthogonal matrix, and $A = U^\top D U$, where $D$ is a fixed positive diagonal matrix. Suppose that $\calA$ is an Adaptive Deterministic Algorithm that generate extended oracle queries $v_1, \dots, v_{K}$, and after the $k$th query knows $A^i v_j$ for all $i+j \le k+1, i \ge 0, 1 \le j \le k$.    
    For any integer $m \ge 1$, let $k$ be the integer such that $\frac{k(k+1)}{2} \le m < \frac{(k+1)(k+2)}{2},$ i.e., $m$ is at least the $k$th triangular number but less than the $(k+1)$th triangular number.
    Consider the order of vectors $v_1, A v_1, v_2, A^2 v_1, A v_2, v_3, A^3 v_1, \dots$ (this enumerates $A^i v_j$ in order of $i+j$, breaking ties with smaller values of $j$ first).
    Let $W_m$ be the set of first $m$ of these vectors and $X_k$ be the set $\{v_1, \dots, v_k\}$. Let $V$ be a Haar-random orthogonal matrix fixing $W_m$ and acting on the orthogonal complement $W_m^\perp$. Then, $(X_k, U) \eqdist (X_k, U V)$.
\end{lemma}

Before proving this lemma, we note that since the algorithm is deterministic and $D$ is fixed, $W_m$ and $X_k$ are deterministic functions of $A$, and thus of $U$. Hence, we can write $v_k(U'), W_m(U'), X_k(U')$ to be the $v_k, W_m, X_k$ that would have been generated if we started with $A' = (U')^\top D U'$. (If no argument is given, $v_k, W_m, X_k$ are assumed to mean $v_k(U), W_m(U), X_k(U)$, respectively.) We note the following proposition.

\begin{proposition} \label{prop:invariant}
    Suppose that $V$ is any orthogonal matrix fixing $W_m$. Then, $W_m(U) = W_m(UV)$.
\end{proposition}

\begin{proof}
    We prove $W_{m'}(U) = W_{m'}(UV)$ for all $m' \le m$. The base case of $k = 1$ is trivial, since $v_1$ is fixed. We now prove the induction step for $m'$.
    
    If $m' \le m$ is a triangular number, $m' = \frac{k(k+1)}{2}$, then the $m'$th vector in $W_m$ is $v_k$. But note that $v_k(U)$ is a deterministic function of $W_{m'-1}(U)$, and $v_k(UV)$ is the same deterministic function of $W_{m'-1}(UV)$. Hence, if the induction hypothesis holds for $m'-1$, it also holds for $m$.

    If $m' \le m$ is not a triangular number, then the $m'$th number in $W_m(U)$ is $A^i v_j$ for some $i \ge 1$. Likewise, the $m'$th number in $W_m(UV)$ is $V^\top A^i V \cdot v_j(UV)$. Since $i \ge 1$, we know that $v_j(U) = v_j(UV)$, by the induction hypothesis on $\frac{j(j+1)}{2} < m'$. But, we know that $V$ fixes $W_m$, which means it fixes $v_j$ and $A^i v_j$. Thus, $V^\top A^i V v_j(UV) = V^\top A^i V v_j = A^i v_j$.
\end{proof}

We are now ready to prove Lemma \ref{lem:random_rotation_fixed_subspace}.

\begin{proof}[Proof of Lemma~\ref{lem:random_rotation_fixed_subspace}]
    We prove this by induction on $m$. For the base case $m = 1$, $U$ is a random matrix and $V$ is a random matrix that fixes $v_1$. Note that $v_1$ is chosen independently of $A$ (and thus of $U$), so $U$ and $V$ are independent. Even for any fixed $V$, the distribution $U V$ is a uniformly random orthogonal matrix, so overall $U \eqdist U V$. Also, $v_1$ is deterministic, so $(v_1, U) \eqdist (v_1, U V)$.
    
    For the induction step, we first focus on the case when $m$ is a triangular number, which means that the $m$th vector added is $v_k$ where $m = \frac{k(k+1)}{2}$. Let $V_1$ be a random orthogonal matrix fixing $W_{m-1}$ and $V_2$ be a random orthogonal matrix fixing $W_m$. Our goal is then to show $(X_k, U) \eqdist (X_k, U V_2)$.
    %Our goal is to show that the marginal distribution of $U V_2$, regardless of the adaptive algorithm's queries, is uniform. 
    %We show that $(X_k, U V_2) \eqdist (X_k, U V_1 V_2) \eqdist (X_k, U V_1) \eqdist (X_k, U)$, where the inductive hypothesis is $(X_{k-1}, U) \eqdist (X_{k-1}, U V_1)$.
    %By the inductive hypothesis on $m-1$, $(X_{k-1}, U V_1)$ and $(X_{k-1}, U)$ have the same distribution, which means that $U V_2$ is also uniform.

    To make this rigorous, we note an order of generating the random variables. First, we generate $U$ randomly: $W_m$ and $X_k$ are deterministic in terms of $U$. Next, we define $V_1$ to be a random rotation fixing $W_{m-1}$. Finally, we define $V_2$ to be a random rotation fixing $W_m$, where $V_1, V_2$ are conditionally independent on $U$.

    First, we prove that $(X_k, U) \eqdist (X_k, UV_1)$. Note that $U \eqdist UV_1$ by our inductive hypothesis. In addition, since $V_1$ fixes $W_{m-1}$, $W_{m-1}(U) = W_{m-1}(UV_1)$. Since $m = \frac{k(k+1)}{2}$ is a triangular number, $X_k(\cdot)$ is a deterministic function of $W_{m-1}(\cdot)$, which means $X_k(U) = X_k(UV_1)$. Hence, $(X_k, U) \eqdist (X_k(UV_1), UV_1) = (X_k, UV_1)$.
        
    Next, we prove that $(X_k, U V_2) \eqdist (X_k, U V_1 V_2)$. It suffices to prove that 
\[(X_k, U, V_2) \eqdist (X_k, UV_1, V_2).\]
    To do so, we first show that $V_2 = f(U, R)$, where $f$ is a deterministic function and $R$ represents a random orthogonal matrix over $d-dim(W_m)$ dimensions that is independent of $U$. (Recall that $W_m$ is a deterministic function of $U$.) To define $f(U, R)$, we consider some deterministic map that sends each $W_m$ to a set of $d-dim(W_m)$ basis vectors in $W_m^\perp$. We then define $V_2 = f(U, R)$ to act on $W_m^\perp$ using $R$ and the correspondence of basis vectors. Since $W_m$ and $X_k$ are deterministic in terms of $U$, this means $f(U, R)$ is well-defined.
    We will now show that 
\[V_2 = f(U, R) = f(UV_1, R) \hspace{0.5cm} \text{and} \hspace{0.5cm} X_k = X_k(UV_1).\]
    Since $U \eqdist UV_1$ by our inductive hypothesis, $(X_k, U, V_2) \eqdist (X_k(UV_1), UV_1, f(UV_1, R)) = (X_k, UV_1, V_2)$, which completes the proof.
    By Proposition \ref{prop:invariant}, $W_{m-1}(U) = W_{m-1}(UV_1),$ and since $X_k(\cdot)$ is deterministic given $W_{m-1}(\cdot)$ for $m = \frac{k(k+1)}{2}$, $X_k(U) = X_k(UV_1)$. This implies $W_m(U) = W_m(UV_1),$ which means $f(UV_1, R) = f(U, R)$, since $f(\cdot, R)$ only depends on $W_m(\cdot)$ and $R$. This completes the proof.
    
    %By our inductive hypothesis, $UV_1 \eqdist U$ has a uniform distribution, so $(X_k, (U V_1) V_2) \eqdist (X_k, U V_2)$. Also, $(X_k, (U V_1)) \eqdist (X_k, U)$ by our inductive hypothesis.
    
    Next, we show that $(X_k, U V_1 V_2) \eqdist (X_k, U V_1)$. Since we chose the order with $U$ being defined first, we are allowed to condition on $U$. Since $X_k$ is deterministic in terms of $U$, it suffices to show that $V_1 V_2|U \eqdist V_1|U$. Since $W_{m-1}, W_m$ are also deterministic given $U$, note that $V_1$ is a uniformly random orthogonal matrix fixing $W_{m-1},$ and $V_2$ is a random orthogonal matrix fixing $W_{m} \supset W_{m-1}$. Since $V_1$ and $V_2$ are conditionally independent given $U$, this means $V_1 V_2|U$ is a uniformly random orthogonal matrix fixing $W_{m-1}$, so $V_1 V_2|U \eqdist V_1|U$.
    
    In summary, we have that
\begin{align*}
    (X_k, U) &\eqdist (X_k, U V_1) \\
    &\eqdist (X_k, U V_1 V_2) \\
    &\eqdist (X_k, U V_2).
\end{align*}
    
    To finish the induction, we focus on the case where $m$ is not a triangular number. Again, let $V_1$ be a random orthogonal matrix fixing $W_{m-1}$ and $V_2$ be a random orthogonal matrix fixing $W_m$. Our goal is again to show that $(X_k, U) \eqdist (X_k, U V_2)$. 
    %This time, we show that $(X_k, U V_2) \eqdist (X_k, U V_2 V_1) \eqdist (X_k, U V_1)$.

    First, we again have $(X_k, U V_1) \eqdist (X_k, U)$ by our inductive hypothesis.
    
    Next, we show that $(X_k, U V_2) \eqdist (X_k, U V_2 V_1)$. It suffices to prove that 
\[(X_k, U, V_2) \eqdist (X_k, UV_1, V_1^\top V_2 V_1),\]
    since $(U V_1) (V_1^\top V_2 V_1) = U V_2 V_1$.
    We recall the random variable $R$ and use the same function $V_2 = f(U, R)$.
    Since we have already shown that $U \eqdist UV_1$, this implies that $(X_k, U, V_2) \eqdist (X_k(UV_1), UV_1, f(UV_1, R))$.
    Since $m$ is not triangular, $X_k(\cdot)$ is contained in $W_{m-1}(\cdot)$, so by Proposition \ref{prop:invariant}, $X_k(U) = X_k(UV_1)$. So, we have 
\[(X_k, U, V_2) \eqdist (X_k(UV_1), UV_1, f(UV_1, R)) = (X_k, UV_1, f(UV_1, R)).\]
    %Finally, we note that $f(UV_1, R)|U, V_1 \eqdist V_1^\top f(U, R) V_1|U, V_1$. This is true because if
    Now, if we fix $U$ and $V_1$, $W_{m-1}(UV_1) = W_{m-1}(U)$, but the final vector in $W_m(UV_1)$ will be $V_1^\top A^i V_1 v_j = V_1^\top (A^i v_j)$, if the final vector in $W_m(U)$ is $A^i v_j$. For fixed $U, V_1$, $f(U, R)$ is a random rotation fixing $W_{m-1}$ and $A^i v_j$, but $f(UV_1, R)$ is a random rotation fixing $W_{m-1}$ and $V_1^\top (A^i v_j)$. Since $V_1^\top$ fixes $W_{m-1}$ by how we defined $V_1$, this means that for fixed $U, V_1$, $f(U, R)$ is a random rotation fixing $W_m$ but $f(UV_1, R)$ is a random rotation fixing $V_1^\top W_m$. Therefore, conditioned on $U, V_1$, $f(UV_1, R)$ has the same distribution as $V_1^\top f(U, R) V_1$. Since $X_k$ is deterministic in terms of $U$, this means
\[(X_k, UV_1, f(UV_1, R))|U, V_1 \eqdist (X_k, UV_1, V_1^\top f(U, R) V_1)|U, V_1.\]
    We can remove the conditioning to establish that $(X_k, UV_1, f(UV_1, R)) \eqdist (X_k, UV_1, V_1^\top f(U, R) V_1) = (X_k, UV_1, V_1^\top V_2 V_1),$ which completes the proof.
        
    Next, we show that $(X_k, U V_2 V_1) \eqdist (X_k, U V_1)$. The proof is essentially the same as in the case when $m$ is triangular. We again condition on $U$, and we have that $V_2 V_1|U \eqdist V_1|U$ have the same distribution as uniform orthogonal matrices fixing $W_{m-1}(U)$. Since $X_k$ is a deterministic function of $U$, this means $(X_k, U V_2 V_1)|U \eqdist (X_k, U V_1)|U,$ and removing the conditioning finishes the proof.
    
    In summary, 
\begin{align*}
    (X_k, U) &\eqdist (X_k, U V_1) \\
    &\eqdist (X_k, U V_2 V_1) \\
    &\eqdist (X_k, U V_2). \qedhere
\end{align*}
\end{proof}

We now prove our main conditioning lemma, which will be a modification of Lemma \ref{lem:random_rotation_fixed_subspace}.

\begin{lemma}[Conditioning Lemma] \label{lem:conditioning_lemma}
    Let all notation be as in Lemma \ref{lem:random_rotation_fixed_subspace}, and let $V_0$ be a fixed orthogonal matrix fixing $W_m$. Importantly, $V_0$ is a deterministic function only depending on $W_m$ (and not directly on $U$). Then, $(X_k, U) \eqdist (X_k, UV_0)$.
\end{lemma}

\begin{proof}
    First, note that since $V_0$ is a deterministic function of $W_m$, it is also a deterministic function of $U$. We can write $V_0(\cdot)$ as this function, and $V_0 = V_0(U)$.

    Now, Lemma \ref{lem:random_rotation_fixed_subspace} proves that $(X_k, U) \eqdist (X_k, UV)$. Note that conditioned on $U$, $V$ is a random matrix fixing $W_m$ and $V_0$ is a fixed matrix fixing $W_m$, which means that $VV_0|U \eqdist V|U$. Hence, $(X_k, UV) \eqdist (X_k, UVV_0)$. But from Proposition \ref{prop:invariant}, $X_k(UV) = X_k(U)$ and $W_m(UV) = W_m(U)$, which means that $V_0(\cdot)$, which only depends on $W_m(\cdot)$, satisfies $V_0(UV) = V_0(U)$. Hence, because $U \eqdist UV$, we have $(X_k, UVV_0) = (X_k(UV), UV \cdot V_0(UV)) \eqdist (X_k(U), U \cdot V_0(U)) = (X_k, UV_0)$.

    In summary, we have that $(X_k, U) \eqdist (X_k, UV) \eqdist (X_k, UVV_0) \eqdist (X_k, UV_0)$, which completes the proof.
\end{proof}

\subsection{From Query Algorithms to Block Krylov Algorithms}\label{scn:from_query}

%In this section, we carry out the high-level outline from Section~\ref{scn:block_kry_overview}. We start by describing the stronger oracle model.

We now aim to prove the following result, which implies that any adaptive deterministic algorithm in the extended oracle model can be simulated by rotating the output of a block Krylov algorithm.

\begin{lemma}[reduction to block Krylov]\label{lem:chen_block_krylov}
    Let $v_1, v_2(\cdot), \dotsc, v_{K}(\cdot)$\todo{explain $v_2(\cdot)$ notation} be an adaptive deterministic algorithm that makes $K$ queries, where $K^2 < d$. Let $\valg_1, \valg_2, \dotsc, \valg_{K}$ be recursively defined as follows: $\valg_1 = v_1$, and $\valg_k = v_k(\{A^i \valg_j\}_{H_{k-1}})$\todo{Explain again what $\{A^i \valg_j\}_{H_{k-1}}$ means} for $k \ge 2$. Let $z_1, \dotsc, z_{K}$ be i.i.d.\ standard Gaussian vectors. Then, from the collection $\{A^i z_j\}_{i+j \le K}$, we can construct a set of unit vectors $\vsim_1,\vsim_2, \dotsc, \vsim_{K}$, and a set of rotation matrices $\Usim_1, \Usim_2, \dotsc, \Usim_{K}$, with the following properties.
\begin{enumerate}
    \item $\vsim_k$ and $\Usim_k$ only depend on $\{A^i z_j\}_{i+j \le k}$. Moreover, $\vsim_k \in \Span(\{A^i z_j\}_{i+j \le k}).$
    \item $\big((\Usim_{1:K})^\top A (\Usim_{1:K}), \{(\Usim_{1:K})^\top A^i \vsim_j\}_{H_{K}}\big) \eqdist \big(A, \{ A^i \valg_j \}_{H_{K}}\big)$, where $\Usim_{1:K} \deq \Usim_1 \dotsm \Usim_{K}$. \todo{clarify that $\eqdist$ means over the randomness of $A$ and $\tilde{z}_i$}\ainesh{rhs is the adaptive algorithm, this statement says that if the adaptive algorithm finds a good subspace, then the simulator finds this too.  }
\end{enumerate}
\end{lemma}

%The proof of the lemma requires introducing a hefty amount of notation, but we emphasize that it follows along the lines of Section~\ref{scn:block_kry_overview}.

First, we describe how to construct $\vsim_k$. Let $\vsim_1 = \frac{z_1}{\norm{z_1}}$, and for $k \ge 2$, let $\vsim_k$ be the unit vector parallel to the component of $z_k$ that is orthogonal to the span of $\{A^i z_j\}_{H_{k-1}}$. (With probability $1$, this is well-defined.) \ainesh{ let $Q_k$ be a basis for $\textrm{ span} \{A^i z_j\}_{H_{k-1}}$. Let $\vsim_k = \Paren{I- Q_k Q_k^\top} v_k  / \norm{ \Paren{I- Q_k Q_k^\top} v_k}_2 $.  }
%\todo{To make sure, $\tilde v_k$ is normalized to be a unit vector? \chen{does that matter? they just have to be orthogonal right? }No you need to make sure an orthogonal matrix can actually send some vector to some other vector, ok its fixed now}. thanks! 
Clearly, $\vsim_k$ is a linear combination of $\{A^i z_j\}_{H_{k-1}}$ and $z_k$, so it is a linear combination of $\{A^i z_j\}_{i+j \le k}$.Therefore, we can construct the set $\{A^i \vsim_j\}_{H_k}$ as a linear combination of the set $\{A^i z_j\}_{H_k}$, for all $k \le K$. The reverse is also true by induction: it clearly holds for $k = 1$, and if it holds for $k-1$, then $z_{k}$ is a linear combination of $\tilde{v}_{k}$ and $\{A^i z_j\}_{H_{k-1}}$. Thus, $z_k$ is a linear combination of $\tilde{v}_k$ and $\{A^i \tilde{v}_j\}_{H_{k-1}}$ by the inductive hypothesis, so $\{A^i z_j\}_{H_k}$ is a linear combination of $\{A^i \tilde{v}_j\}_{H_k}$.

\ainesh{make the above a tiny lemma.}

\ainesh{make this a definition.}
To construct the rotation matrices $\Usim_k$, we will first define matrix-valued functions $U_k(\cdot)$, for $k=1, \dots, K$, which takes arguments $\{x_{i,j}\}_{H_{k-1}}$, $y$, $z$, where the vectors $y$ and $z$ have unit norm and are both orthogonal to the collection $\{x_{i,j}\}_{H_{k-1}}$. Since $H_{0}$ is empty, the first function $U_1$ only takes arguments $y_1, z_1$, and is such that $U_1(y_1, z_1)$ is a deterministic orthogonal matrix that satisfies $U_1(y_1, z_1)^\top y_1 = z_1$. This is possible because $y_1$ and $z_1$ both have unit norm; for example, we can complete $y_1$ and $z_1$ to orthonormal bases $(y_1,y_2,\dotsc,y_{d})$, $(z_1,z_2,\dotsc,z_{d})$ and take $U_1(y_1,z_1) = \sum_{i=1}^{d} y_i z_i^\top$.
%For $k>1$, let 
%\begin{align*}
%    M_l = U_l(\{x_{i,j}\}_{i+j\le l, j<l}, \{y_j\}_{j\le l}, \{z_j\}_{j\le l})\, , \, \forall l \le k-1\,,
%\end{align*}
Next, $U_k(\{x_{i,j}\}_{H_{k-1}}, y_k, z_k)$ is a deterministic orthogonal matrix that satisfies
\begin{align}
\begin{aligned}\label{eq:uk_func}
    U_k^\top x_{i,j} &= x_{i,j}\,, \qquad \text{for all}~ (i, j) \in H_{k-1}\,, \\
    U_k^\top y_k &= z_k\,.
\end{aligned}
\end{align}
Such a choice of $U_k$ is always possible, because $k^2 < d$, and because $y_k$ and $z_k$ are orthogonal to $x_{i,j}$; for example, we can start with the identity matrix on the subspace spanned by $\{x_{i,j}\}_{H_{k-1}}$ and add to it a sum of outer products formed by completing $y_k$ and $z_k$ to two orthonormal bases of the orthogonal complement.


\ainesh{think of $v_k^{sim}$ to be the vectors that the simulator thinks the algorithm is querying. Think of $U_k^{sim}$ to be the rotations that keep the distribuition on the orthogonal complement of everything so far remains rotationally invariant. }
Next, we describe how to construct $\Usim_k$. We first need to construct an auxiliary sequence $\{\vssim_k\}_{k=1,2,\dotsc,K-1}$. We let $\vssim_1 = v_1$, and $\Usim_1 = U_1(\vsim_1, \vssim_1)$. For $k \ge 2$, $\vssim_k$ and $\Usim_k$ are defined recursively as follows:
\begin{align}
\begin{aligned}\label{eq:vs_us}
    \vssim_k &= v_k\bigl(\{(\Usim_{1:(k-1)})^\top A^i \vsim_j\}_{H_{k-1}}\bigr)\\
    \Usim_k &= U_k\bigl(\{(\Usim_{1:(k-1)})^\top A^i \vsim_j\}_{H_{k-1}},\; (\Usim_{1:(k-1)})^\top \vsim_k,\; \vssim_k\bigr)\, .
\end{aligned}
\end{align}
%\todo{last argument above is $v_j^{(s)}$ right?}
\todo{make $\vssim$ and $\Usim$ a definition, and $\Usim$ is well defined a lemma}
To show that this choice of $\Usim_k$ is possible, we need to check that $(\Usim_{1:(k-1)})^\top \vsim_k$, $\vssim_k$ both have unit norm and are orthogonal to the subspace $S_k$ spanned by $(\Usim_{1:(k-1)})^\top A^i \vsim_j$ for $(i, j) \in H_{k-1}$. They both have unit norm because $\vsim_k$ and $\vssim_k$ are constructed to have unit norm, and inductively we can assume $\Usim_{1:(k-1)}$ is orthogonal. Note that $\vssim_k$ is orthogonal to $S_k$ by our assumption on the function $v_k(\cdot)$, and $(\Usim_{1:(k-1)})^\top \vsim_k$ is also orthogonal to $S_k$ because
\begin{align*}
    \langle (\Usim_{1:(k-1)})^\top A^i \vsim_j, (\Usim_{1:(k-1)})^\top\vsim_k\rangle = \langle A^i \vsim_j, \vsim_k\rangle = 0\, ,
\end{align*}
where the second line follows from the definition of $\tilde v_k$.

%Such choices of $U^{(s)}_k$ is possible for all $k^2 \le d$. In addition, to see why $U_k^{(s)}$ can be orthogonal, note it fixes the $x_{i, j} = \{(U_{1:(k-1)}^{(s)})^\top A_0^i \tilde{v}_j\}$ vectors for $i+j \le K, j < K$, and it sends $y_k = (U_{1:(k-1)}^{(s)})^\top \tilde{v}_k$ to $v_k^{(s)}$, which are both unit vectors by construction (and inductively assuming $U_1^{(s)}, \dots, U_{k-1}^{(s)}$ are orthogonal). In addition, by the orthogonality constraints of $\tilde{v}_k$, $y_k$ is orthogonal to every $x_{i, j},$ and also $v_k^{(s)}$, by definition, is orthogonal to every $x_{i, j}$ for $i+j \le k, j < k$. Hence, we can choose $U_k^{(s)}$ to be orthogonal. \todo{To Chen: i explained why $U_k^{(s)}$ is orthogonal }\chen{yeah looks good. i might move this to the definition of the function $U_k$ later} 

 We summarize some important additional properties of $\vssim_k$ and $\Usim_k$ in the following lemma.
\begin{lemma}[Properties of the Simulated Sequences]\label{lem:krylov_aux}
The variables $\Usim_k$ and $\vssim_k$ for $k = 1, \dotsc, K$ defined above satisfy the following properties:
\begin{enumerate}[label=(P\arabic*), ref=(P\arabic*)]
\item \label{prop1} $\vssim_k$ and $\Usim_k$ depend only on $\{A^i \vsim_j\}_{i+j \le k}$. \ainesh{randomness in the simulator so far only depends on the randomness in the queries so far.}
\item \label{prop2} \ainesh{simulator is indeed simulating algorithm queries.} For any $k \ge j$, we have
\begin{align*}
    \vsim_j = \Usim_{1:k} \vssim_j\, .
\end{align*}
\item \label{prop3} \todo{quantify $k$. $k$ at least 2?} \ainesh{invoking def }  $\vssim_k$ satisfies
\begin{align*}
    \vssim_k
    &= v_k\bigl(\{(\Usim_{1:(k-1)})^\top A^i \Usim_{1:(k-1)} \vssim_j\}_{H_{k-1}}\bigr)\,.
    %&= v_k\bigl(((\Usim_{1:(K-1)})^\top A^i \Usim_{1:(K-1)} \vssim_j)_{i+j<k}\bigr)\,.
\end{align*}
\item \label{prop4} $\Usim_k$ satisfies
\begin{align*}
    \Usim_k &= U_k\bigl(\{(\Usim_{1:(k-1)})^\top A^i \Usim_{1:(k-1)}\vssim_j\}_{H_{k-1}},\; (\Usim_{1:(k-1)})^\top \vsim_k,\; \vssim_k\bigr)\, .
\end{align*}
\end{enumerate}
\end{lemma}
\begin{proof}
    \ref{prop1} is immediate from the definitions, since $\{(i, j): i+j \le k\} = H_{k-1} \cup \{(0, k)\}$. 
    
    To show \ref{prop2}, note that the second property of the function $U_k$ from \eqref{eq:uk_func} implies that
    \begin{align}\label{eq:tildev}
         \vssim_j = (\Usim_j)^\top (\Usim_{1:(j-1)})^\top\vsim_j = (\Usim_{1:j})^\top\vsim_j\, . 
    \end{align}
    This proves~\ref{prop2} for $k = j$. To prove~\ref{prop2} for $k > j$, we use induction on $k$. If~\ref{prop2} holds for $k-1 \ge j$, then
    \begin{align}
        (\Usim_{1:k})^\top \vsim_j = (\Usim_k)^\top (\Usim_{1:(k-1)})^\top \vsim_j = (\Usim_{1:(k-1)})^\top \vsim_j = \vssim_j.
    \end{align}
    Above, the middle equality holds by the first property of \eqref{eq:uk_func}, since $\Usim_k$ fixes $(\Usim_{1:(k-1)})^\top \vsim_j$ because $j \le k-1$. The final equality holds by our inductive hypothesis. So, \ref{prop2} holds for $k$.
    
    Finally, \ref{prop3} and \ref{prop4} then follow from~\ref{prop2}, since $k-1 \ge j$ if $j \in H_{k-1}$. %, as well as the definition of $\Usim_k$.
\end{proof}

We are now ready to prove Lemma~\ref{lem:chen_block_krylov}.
Although the proof is notationally burdensome, the message is that we can show the equality of distributions inductively by repeatedly invoking the conditioning lemma (Lemma~\ref{lem:conditioning_lemma}), which is designed precisely for the present situation.

\medskip

\begin{proof}[Proof of Lemma~\ref{lem:chen_block_krylov}]

It is clear that $\vsim_1, \dots, \vsim_K$ and $\Usim_1, \dots, \Usim_K$ satisfy Property 1 in Lemma \ref{lem:chen_block_krylov}. 
We focus on proving the second property.
For $1 \le k \le K$, let $A_{k} \deq (\Usim_{1:k})^\top A \Usim_{1:k}$.
Since we can write $(\Usim_{1:k})^\top A^i \vsim_j = (\Usim_{1:k})^\top A^i (\Usim_{1:k}) \vssim_j = A_k^i \vssim_j$ for any $k \ge j$ by~\ref{prop2} of Lemma \ref{lem:krylov_aux}, it suffices to inductively prove that for all $1 \le k \le K$, 
    \begin{align} \label{eq:goal2}
        (A_k, \{\vssim_j\}_{1 \le j \le k}) \eqdist (A, \{\valg_j\}_{1 \le j \le k}).
    \end{align}
    %\eqref{eq:goal2} implies \eqref{eq:goal} because $\{A_{K-1}^i \vssim_j\}_{H_{K-1}}$ is a deterministic function of $(A_{K-1}, \{\vssim_j\}_{1 \le j \le K-1})$ and $\{A^i \valg_j\}_{H_{K-1}}$ is the same deterministic function of $(A, \{\valg_j\}_{1 \le j \le K-1})$.

    For the base case of $k = 1$, it suffices to show that $(A_1, \vssim_1) \eqdist (A, \valg_1)$. Note, however, that $\vssim_1 = \valg_1 = v_1$, and $A_1 = (\Usim_1)^\top A (\Usim_1) = U_1(\vsim_1, v_1)^\top A U_1(\vsim_1, v_1)$.
    Since $v_1$ is a deterministic vector, $\vsim_1$ is independent of $A$, and the distribution of $A$ is rotationally invariant, the claim follows.

    For the inductive step, assume we know $(A_k, \{\vssim_j\}_{1 \le j \le k}) \eqdist (A, \{\valg_j\}_{1 \le j \le k})$. Then, note that $\valg_{k+1} = v_{k+1}(\{A^i \valg_j\}_{H_k})$ and $\vssim_{k+1} = v_k(\{A_k^i \vssim_j\}_{H_k})$. Therefore, we can write $\valg_{k+1} = \mathfrak{D}_{k+1}(A, \{\valg_j\}_{1 \le j \le k})$ and $\vssim_{k+1} = \mathfrak{D}_{k+1}(A_k, \{\vssim_j\}_{1 \le j \le k})$, for the same deterministic function $\mathfrak{D}_{k+1}$. In addition, because $\Usim_{k+1}$ fixes $A_k^i \vssim_j$ for all $(i, j) \in H_k$ by~\ref{prop4}, we also have that $A_{k+1}^i \vssim_j = A_k^i \vssim_j$ for all $(i, j) \in H_k$, which means $\vssim_{k+1} = \mathfrak{D}_{k+1}(A_{k+1}, \{\vssim_j\}_{1 \le j \le k})$ for the same $\mathfrak{D}_{k+1}$. Therefore, it suffices to show 
    \begin{align} \label{eq:goal3}
        (A_{k+1}, \{\vssim_j\}_{1 \le j \le k})
        \eqdist (A, \{\vssim_j\}_{1 \le j \le k})\,,
    \end{align}
    as this implies $(A_{k+1}, \{\vssim_j\}_{1 \le j \le k+1}) \eqdist (A, \{\valg_j\}_{1 \le j \le k+1})$, which completes the inductive step.

    \ainesh{next we show that if you are a random vector orthgonal to the queries of the alg so far, then you are a random vector orthgonal to the simulated querires so far.}
    Note that $A_{k+1} = (\Usim_{k+1})^\top A_k (\Usim_{k+1})$, where,  by~\ref{prop4},
    \begin{equation} \label{eq:Usim_k+1_redefined}
        \Usim_{k+1} = U_{k+1}(\{A_k^i \vssim_j\}_{H_k}, (\Usim_{1:k})^\top\tilde{v}_{k+1}, \vssim_{k+1}).
    \end{equation}
   Note that $\tilde{v}_{k+1}$ is a random unit vector orthogonal to $\{A^i z_j\}_{H_k}$, or equivalently, it is a random unit vector orthogonal to $\{A^i \vsim_j\}_{H_k}$. However, since $(\Usim_{1:k})^\top A^i \vsim_j = (\Usim_{1:k})^\top A^i(\Usim_{1:k}) \vssim_j = A_k^i \vssim_j$ for all $(i, j) \in H_k$ (by~\ref{prop2}), this means that $(\Usim_{1:k})^\top \vsim_{k+1}$ is a random unit vector orthogonal to $\{A_k^i \vssim_j\}_{H_k}$. 
    
    Recalling that $\vssim_{k+1} = \mathfrak{D}_{k+1}(A_{k}, \{\vssim_j\}_{1 \le j \le k})$, this means that we can rewrite \eqref{eq:Usim_k+1_redefined} as
    \begin{align*}
        \Usim_{k+1} =& \hspace{0.1cm} U_{k+1}\left(\{A_k^i \vssim_j\}_{H_k}, \hat{v}^{\msf{sim}}, \mathfrak{D}_{k+1}(A_{k}, \{\vssim_j\}_{1 \le j \le k})\right), \\
    \intertext{where $\hat{v}^{\msf{sim}}$ is a random unit vector orthogonal to $\{A_k^i \vssim_j\}_{H_k}$.
    As a result, if we define}
        U_{k+1}^{\msf{alg}} \deq& \hspace{0.1cm} U_{k+1}\left(\{A^i \valg_j\}_{H_k}, \hat{v}^{\msf{alg}}, \mathfrak{D}_{k+1}(A, \{\valg_j\}_{1 \le j \le k})\right),
    \end{align*}
    where $\hat{v}^{\msf{alg}}$ is a random unit vector orthogonal to $\{A^i \valg_j\}_{H_k}$, then 
    \begin{align*}
        (A_{k+1}, \{\vssim_j\}_{1 \le j \le k}) &= ((\Usim_{k+1})^\top A_k (\Usim_{k+1}), \{\vssim_j\}_{1 \le j \le k}) \\
        &\eqdist \left((U_{k+1}^{\msf{alg}})^\top A (U_{k+1}^{\msf{alg}}), \{\valg_j\}_{1 \le j \le k}\right).
    \end{align*}
    Above, the first equality follows by definition, and the third follows from our inductive hypothesis that $(A_k, \{\vssim_j\}_{1 \le j \le k}) \eqdist (A, \{\valg_j\}_{1 \le j \le k}).$

    \ainesh{add more exposition below, including def of $\cal{D}$.}
    We are now in a position to apply the conditioning lemma (Lemma~\ref{lem:conditioning_lemma}).
    Note that $U_{k+1}^{\msf{alg}}$ only depends on $\{A^i \valg_j\}_{H_k}$ (as well as some randomness in $\hat{v}^{\msf{alg}}$, but the randomness is independent of everything else given $\{A^i \valg_j\}_{H_k}$, so we can safely condition on it). Hence, we can apply the conditioning lemma with $U_{k+1}^{\msf{alg}}$, to obtain that 
    \begin{align*}
        (A_{k+1}, \{\vssim_j\}_{1 \le j \le k}) \eqdist \left((U_{k+1}^{\msf{alg}})^\top A (U_{k+1}^{\msf{alg}}), \{\valg_j\}_{1 \le j \le k}\right) \eqdist \left(A, \{\valg_j\}_{1 \le j \le k}\right) \,,
    \end{align*}
    which establishes \eqref{eq:goal3} and thereby concludes the proof.
\end{proof}

\subsection{General Matrix-Vector Lower Bound}

We are now ready to combine the information-theoretic lower bound against Block Krylov algorithms and our lifting statement that shows Block Krylov can simulate an Adaptive  Detereministic Algorithm (see Def~\ref{def:adaptive-deterministic-algorithm}) to obtain an information-theoretic lower bound on the number of matrix-vector products.  

\begin{theorem}[Matrix-Vector Lower Bound for Spectral LRA]
    Fix $D$ as in Definition \ref{def:hard-distribution-chebyshev-polynomial}. Any (potentially randomized) adaptive algorithm on the distribution $A = U^\top D U$ cannot output a unit vector $v$ such that $\langle v, u_1(A) \rangle \ge \sqrt{\frac{\eps}{3}},$ with more than $0.2$ probability over the randomness of both $A$ and the algorithm.
    Here, $u_1(\cdot)$ represents the maximum eigenvector of a symmetric matrix.
    Hence, by Proposition \ref{prop:correlated-with-top-eigvec}, outputting a $(1+\eps)$-approximate rank-1 approximation to $A$ with more than $0.4$ probability needs $\Omega\left(\frac{\log n}{\sqrt{\eps}}\right)$ adaptive queries.
\end{theorem}

\begin{proof}
    First we assume that the algorithm is deterministic, so its behavior is characterized by functions $v_1, v_2(\cdot), \dotsc, v_K(\cdot)$, as in Lemma~\ref{lem:chen_block_krylov}.
    Using one additional query $v_{K+1}(\cdot)$, the algorithm can ensure that some linear combination of $v_{K+1}$ and $\{A^i v_j\}_{H_K}$ contains such a vector $v$ with at least $0.2$ probability. So, our goal is to show that $\Span(\{A^i \valg_j\}_{i+j \le K+1})$ cannot contain such a vector $v$ with high probability.

    By Lemma \ref{lem:chen_block_krylov}, a block Krylov algorithm that receives $\{A^i z_j\}_{i+j \le K+1}$ can generate $\tilde{v}_1, \dots, \tilde{v}_{K+1},$ where each $\tilde{v}_k \in \Span(\{A^i z_j\}_{i+j \le k})$, along with $\Usim_1, \dots, \Usim_{K+1}$, so that 
\[\big((\Usim_{1:(K+1)})^\top A (\Usim_{1:(K+1)}), \{(\Usim_{1:(K+1)})^\top A^i \vsim_j\}_{H_{K+1}}\big) \eqdist \big(A, \{ A^i \valg_j \}_{H_{K+1}}\big).\]
    Then, if with at least $0.2$ probability there exists a unit vector $v \in \Span(\{A^i \valg_j\}_{i+j \le K+1})$ with $\langle v, u_1(A) \rangle \ge \sqrt{\frac{\eps}{3}}$, then with the same probability there exists a unit vector 
\[v' \in \Span(\{U_{1:(K+1)}^\top A^i \tilde{v}_j\}_{i+j \le K+1}) = U_{1:(K+1)}^\top \cdot \Span(\{A^i z_j\}_{i+j \le K+1})\]
    with $\big\langle v', u_1\big((\Usim_{1:(K+1)})^\top A (\Usim_{1:(K+1)})\big)\big\rangle \ge \sqrt{\frac{\eps}{3}}$. However, the top eigenvector of $(\Usim_{1:(K+1)})^\top A (\Usim_{1:(K+1)})$ is $(\Usim_{1:(K+1)})^\top u_1(A)$, so this means $\langle v', (\Usim_{1:(K+1)})^\top u_1(A) \rangle \ge \sqrt{\frac{\eps}{3}}.$ In turn, this implies that the span of $\{A^i z_j\}_{i+j \le K+1}$ has a unit vector $v''$ with $\langle v'', u_1(A) \rangle \ge \sqrt{\frac{\eps}{3}}$ with at least $0.2$ probability, which contradicts \Cref{lem:lb-against-krylov-main}. Hence, no deterministic algorithm can succeed with more than $0.2$ probability.

    If the algorithm is randomized, then it uses a random seed $\xi$ that is independent of $A$. So conditional on the random seed, the algorithm will not be able to succeed with more than $0.2$ probability, which means the overall probability that the randomized algorithm successfully finds such a vector is also at most $0.2$.
\end{proof}
